Content-Adaptive Motion Rate Adaption for Learned Video Compression

This paper introduces an online motion rate adaptation scheme for learned video compression, with the aim of achieving content-adaptive coding on individual test sequences to mitigate the domain gap between training and test data. It features a patch-level bit allocation map, termed the $\alpha$-map, to trade off between the bit rates for motion and inter-frame coding in a spatially-adaptive manner. We optimize the $\alpha$-map through an online back-propagation scheme at inference time. Moreover, we incorporate a look-ahead mechanism to consider its impact on future frames. Extensive experimental results confirm that the proposed scheme, when integrated into a conditional learned video codec, is able to adapt motion bit rate effectively, showing much improved rate-distortion performance particularly on test sequences with complicated motion characteristics.

==> chapter/4-1_rd.tex <==
\begin{figure*}[h]
\begin{center}
\begin{subfigure}{0.39\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \hspace{-2em}
    \includegraphics[width=0.9\linewidth]{figure/UVG_13.png}
    \vspace{-0.6em}
    \caption{UVG, PSNR}
    %\vspace{-1.2em}
    \label{fig:uvgPSNR}
\end{subfigure}%\hspace{-2em}%\hfill
\begin{subfigure}{0.39\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \includegraphics[width=0.9\linewidth]{figure/HEVCB_13.png}
    \vspace{-0.6em}
    \caption{HEVC Class B, PSNR}
    %\vspace{-1.2em}
    \label{fig:hevcPSNR}
\end{subfigure}%\hspace{2em}

\begin{subfigure}{0.39\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \hspace{-2em}
    \includegraphics[width=0.9\linewidth]{figure/MCL_13.png}
    \vspace{-0.6em}
    \caption{MCL-JCV, PSNR}
    %\vspace{-1.2em}
    \label{fig:mclPSNR}
\end{subfigure}%\hspace{-2em}%\hfill
\begin{subfigure}{0.39\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \includegraphics[width=0.9\linewidth]{figure/GC_test_13.png}
    \vspace{-0.6em}
    \caption{ISCAS'22 GC, PSNR}
    %\vspace{-1.2em}
    \label{fig:gcPSNR}
\end{subfigure}%\hspace{2em}
\caption{Rate-distortion performance evaluation on UVG, HEVC Class B, MCL-JCV, and ISCAS'22 GC datasets.}
\label{fig:RD}
\end{center}
\vspace{-2.0em}
\end{figure*}

==> chapter/4-2-2_bd_rate_noDCVC.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\vspace{5cm}
\begin{table}[]
\vspace{5cm}
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{ID}} & \multicolumn{2}{c}{\textbf{BD-rate (\%) PSNR}} \\ \cline{3-4} 
                                   &                              & \textbf{Ours$^1$}      & \textbf{Ours$^2$}     \\ \hline
\multirow{7}{*}{\textbf{UVG$^*$}}  & \textbf{Beauty}              & -2.49                  & -2.77                 \\
                                   & \textbf{Bosphorus}           & -2.12                  & -2.60                 \\
                                   & \textbf{HoneyBee}            & -1.36                  & -1.51                 \\
                                   & \textbf{Jockey}              & -4.30                  & -4.61                 \\
                                   & \textbf{ReadySteadyGo}       & -3.89                  & -4.07                 \\
                                   & \textbf{ShakeNDry}           & -0.68                  & -1.40                 \\
                                   & \textbf{YachtRide}           & -3.12                  & -3.28                 \\ \hline
\multirow{4}{*}{\textbf{HEVC-D}}   & \textbf{BasketballPass}      & -2.16                  & -3.17                 \\
                                   & \textbf{BlowingBubbles}      & -3.27                  & -3.19                 \\
                                   & \textbf{BQSquare}            & -2.47                  & -2.66                 \\
                                   & \textbf{RaceHorses}          & -3.39                  & -3.32                 \\ \bottomrule
\end{tabular}
\end{table}

==> chapter/4-3_lambda_table.tex <==
\begin{table}[]
\vspace{1em}
\centering
\caption{$\lambda_I$ and $\lambda_P$ for variable-rate encoding.} 
\label{tab:lambda_range}
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|}
\hline
$\lambda_P$ & 1024                   & 4096                   & 16384                  & 65536                  \\ \hline
$\lambda_I$ & $5e^{-3} \sim 5e^{-2}$ & $1e^{-2} \sim 1e^{-1}$ & $2e^{-2} \sim 2e^{-1}$ & $2e^{-1} \sim 5e^{-1}$ \\ \hline
\end{tabular}
}
\vspace{-2em}
\end{table}


==> chapter/4-4_flow.tex <==
\begin{figure}[h]
\begin{center}
\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \hspace{-2em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_ref_frame_step_332.png}
    \caption{reference frame}
    %\vspace{-1.2em}
    \label{fig:ref_frame}
\end{subfigure}%\hspace{-2em}%\hfill
\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_gt_frame_step_332.png}
    \caption{current frame}
    %\vspace{-1.2em}
    \label{fig:gt_frame}
\end{subfigure}%\hspace{2em}

\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \hspace{-2em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_flow_map_step_99.png}
    \caption{optical flow before overfit}
    %\vspace{-1.2em}
    \label{fig:flow_99}
\end{subfigure}%\hspace{-2em}%\hfill
\begin{subfigure}{0.44\linewidth}
    % include first image
    \centering
    %\vspace{-0.8em}
    \includegraphics[width=0.9\linewidth]{figure/flow maps/ISCAS_Grand_Challenge_Validation5_flow_map_step_332.png}
    \caption{optical flow after overfit}
    %\vspace{-1.2em}
    \label{fig:flow_332}
\end{subfigure}%\hspace{2em}
\caption{\color{red}Optical flow comparison on the interlaced sequence.}
\label{fig:flow}
\end{center}
\vspace{-2.0em}
\end{figure}

==> chapter/6_Reference.tex <==
\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}
\color{red}
IEEE conference templates contain guidance text for composing and formatting conference papers. Please ensure that all template text is removed from your conference paper prior to submission to the conference. Failure to remove the template text from your paper may result in your paper not being published.


==> chapter/Z_Acknowledgment.tex <==

\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.
